An accurate and efficient framework for modelling the surface chemistry of ionic materials

Quantum-mechanical simulations can offer atomic-level insights into chemical processes on surfaces. This understanding is crucial for the rational design of new solid catalysts as well as materials to store energy and mitigate greenhouse gases. However, achieving the accuracy needed for reliable predictions has proven challenging. Density functional theory (DFT), the workhorse quantum-mechanical method, can often lead to inconsistent predictions, necessitating accurate methods from correlated wave-function theory (cWFT). However, the high computational demands and significant user intervention associated with cWFT have traditionally made it impractical to carry out for surfaces. In this work, we address this challenge, presenting an automated framework which leverages multilevel embedding approaches, to apply accurate cWFT methods to the surfaces of ionic materials with computational costs approaching DFT. With this framework, we have reproduced experimental adsorption enthalpies for a diverse set of 19 adsorbate-surface systems. Moreover, we resolve debates on the adsorption configuration of several systems, while offering benchmarks to assess DFT. This framework is open-source, making it possible to more routinely apply cWFT to complex problems involving the surfaces of ionic materials.

==> Tables/SI_Table-Erlx_MgO.tex <==
\begin{table}
\caption{\label{tab:lattice_parameters_mgo}Relaxation energy $E_\text{rlx}$ (in meV) for the adsorbate--surface systems with the MgO surface obtained from the DFT ensemble.}
\begin{tabular}{lrrrrrr}
\toprule
 & PBE-D2[Ne] & revPBE-D4 & vdW-DF & rev-vdW-DF2 & PBE0-D4 & B3LYP-D2[Ne] \\ 
\midrule
CH$_4$ on MgO(001) & 4 & 2 & 0 & 2 & 0 & 0 \\
Monolayer CH$_4$ on MgO(001) & 3 & 1 & 0 & 2 & -2 & -1 \\
C$_2$H$_6$ on MgO(001) & 3 & 1 & -2 & 2 & -4 & -3 \\
Monolayer C$_2$H$_6$ on MgO(001) & 4 & 4 & 1 & 2 & -4 & -1 \\
CO on MgO(001) & 13 & 8 & 13 & 13 & 9 & 11 \\
C$_6$H$_6$ on MgO(001) & 24 & 26 & 11 & 18 & 6 & 7 \\
Parallel N$_2$O on MgO(001) & 5 & 3 & 4 & 6 & 2 & 4 \\
Tilted N$_2$O on MgO(001) & 9 & 10 & 3 & 11 & 7 & 6 \\
Vertical-Hollow NO on MgO(001) & 75 & 29 & 13 & 62 & 2 & 3 \\
Vertical-Mg NO on MgO(001) & 10 & 9 & 9 & 48 & 5 & 5 \\
Bent-Bridge NO on MgO(001) & 49 & 51 & 33 & 51 & 13 & 9 \\
Bent-Mg NO on MgO(001) & 7 & 6 & 7 & 7 & 2 & 2 \\
Bent-O NO on MgO(001) & 39 & 39 & 18 & 39 & 3 & 5 \\
Dimer NO on MgO(001) & 54 & 42 & 46 & 54 & 20 & 26 \\
Monomer H$_2$O on MgO(001) & 131 & 114 & 90 & 134 & 121 & 113 \\
Tetramer H$_2$O on MgO(001) & 60 & 52 & 51 & 60 & 59 & 58 \\
Tilted CH$_3$OH on MgO(001) & 163 & 145 & 102 & 152 & 141 & 132 \\
Parallel CH$_3$OH on MgO(001) & 48 & 46 & 26 & 43 & 41 & 35 \\
Tetramer CH$_3$OH on MgO(001) & 79 & 68 & 58 & 75 & 69 & 75 \\
NH$_3$ on MgO(001) & 99 & 89 & 103 & 95 & 106 & 115 \\
Physisorbed CO$_2$ on MgO(001) & 15 & 14 & 6 & 16 & 10 & 9 \\
Chemisorbed CO$_2$ on MgO(001) & 693 & 663 & 704 & 676 & 773 & 810 \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/SI_Table-Erlx_TiO2.tex <==
\begin{table}
\caption{\label{tab:lattice_parameters_tio2}Relaxation energy $E_\text{rlx}$ (in meV) for the adsorbate--surface systems with the \ce{TiO2} surfaces obtained from the DFT ensemble.}
\begin{tabular}{lrrrrrr}
\toprule
 & PBE-TS/HI & revPBE-D4 & vdW-DF & rev-vdW-DF2 & r$^2$SCAN-rVV10 & HSE06-D4 \\ 
\midrule
CH$_4$ on TiO$_2$ rutile(110) & 15 & 22 & 5 & 27 & 44 & 26 \\
Parallel CO$_2$ on TiO$_2$ rutile(110) & 25 & 14 & 17 & 30 & 32 & 30 \\
Tilted CO$_2$ on TiO$_2$ rutile(110) & 35 & 50 & 37 & 72 & 92 & 78 \\
H$_2$O on TiO$_2$ rutile(110) & 294 & 238 & 177 & 295 & 320 & 318 \\
CH$_3$OH on TiO$_2$ rutile(110) & 360 & 302 & 266 & 363 & 379 & 390 \\
H$_2$O on TiO$_2$ anatase(101) & 235 & 225 & 157 & 246 & 267 & 257 \\
NH$_3$ on TiO$_2$ anatase(101) & 223 & 212 & 194 & 223 & 237 & 247 \\
\bottomrule
\end{tabular}
\end{table}
